A Framework for Robot Manipulation: Skill Formalism, Meta Learning and Adaptive Control

In this paper we introduce a novel framework for expressing and learning force-sensitive robot manipulation skills. It is based on a formalism that extends our previous work on adaptive impedance control with meta parameter learning and compatible skill specifications. This way the system is also able to make use of abstract expert knowledge by incorporating process descriptions and quality evaluation metrics. We evaluate various state-of-the-art schemes for the meta parameter learning and experimentally compare selected ones. Our results clearly indicate that the combination of our adaptive impedance controller with a carefully defined skill formalism significantly reduces the complexity of manipulation tasks even for learning peg-in-hole with submillimeter industrial tolerances. Overall, the considered system is able to learn variations of this skill in under 20 minutes. In fact, experimentally the system was able to perform the learned tasks faster than humans, leading to the first learning-based solution of complex assembly at such real-world performance.

==> problem_definition.tex <==
\subsection{Controller}\label{sec:pd_controller}

Consider the rigid robot dynamics 
\begin{equation}
{M}(\mathbf{q})\ddot{\mathbf{q}}+{C}(\mathbf{q},\dot{\mathbf{q}})\dot{\mathbf{q}}+\mathbf{g}(\mathbf{q})=\bm{\tau}_u+\bm{\tau}_{ext},
\end{equation}
where ${M}(\mathbf{q})$ denotes the symmetric, positive definite mass matrix, ${C}(\mathbf{q},\dot{\mathbf{q}})\dot{\mathbf{q}}$ the Coriolis and centrifugal torques, $\mathbf{g}(\mathbf{q})$ the gravity vector and $\bm{\tau}_{ext}$ the vector of external link-side joint torques. The adaptive impedance control law is defined as
\begin{equation}
\bm{\tau}_u(t)={J}(\mathbf{q})^T( -\mathbf{F}_{ff}(t)-\V{F}_d(t)-{K}(t)\mathbf{e}-{D}(\bm{q})\dot{\mathbf{e}})+\bm{\tau}_r,
\end{equation}\label{eq:control_law}
where $\mathbf{F}_{ff}(t)$ denotes the adaptive feed-forward wrench, $\V{F}_d (t)$ is an optional initial time dependent feed-forward wrench trajectory, ${K}(t)$ the stiffness matrix, $D$ the damping matrix and ${J}(\mathbf{q})$ the Jacobian.
The position and velocity error are $\mathbf{e}=\V{x}^\star - \V{x}$ and $\dot{\mathbf{e}}=\dot{\V{x}}^\star - \dot{\V{x}}$, respectively. ''${}^\star$" denotes the desired motion command.
The dynamics compensator $\bm{\tau}_r$ can be defined in multiple ways, see for example %\cite{}.
The adaptive tracking error is 
\begin{equation}
\mathbf{\epsilon}=\mathbf{e}+\kappa\dot{\mathbf{e}} ,
\end{equation}
with $\kappa>0$. The adaptive feed forward wrench $\V{F}_{ff}$ is defined as 
\begin{equation}
\V{F}_{ff} = \int_{0}^t  \dot{\boldsymbol{F}}_{ff}(t) \mathrm{d}t + \V{F}_{ff,0}, 
\end{equation}
%where $\V{F}_d (t)$ is an optional initial time dependent trajectory
where $\V{F}_{ff,0}$ is the initial value. The controller adapts feed forward wrench and stiffness by
\begin{align}
\dot{\boldsymbol{F}}_{ff}(t)&=\frac{1}{T}{\alpha}(\boldsymbol{\epsilon}-{\gamma}_\alpha(t)\boldsymbol{F}_{ff}(t))\label{eq:adapt_ff}\\
\dot{K}(t)&=\frac{1}{T}{\beta}(\text{diag}(\boldsymbol{\epsilon}\circ \boldsymbol{e})-{\gamma}_\beta(t){K}(t)). \label{eq:adapt_k}
\end{align}

The positive definite matrices $\alpha$, $\beta$, $\gamma_\alpha$ and $\gamma_\beta$ are the learning rates for feed-forward command and stiffness as well as the respective forgetting factors. The learning rates $\alpha$ and $\beta$ determine stiffness and feed-forward adaptation speed. $\gamma_\alpha$ and $\gamma_\beta$ are responsible for slowing down the adaptation process, which is the main dynamical process for low errors. Cartesian damping ${D}(\bm{q})$ is designed according to \cite{Albu-SchafferOttFreHir2003} and $T$ denotes the sample time of the controller.

Reordering and inserting \eqref{eq:adapt_ff} and \eqref{eq:adapt_k} into \eqref{eq:control_law} leads to a single equation
\begin{equation}
\bm{\tau}_u = f_c (\dot{\mathbf{x}}_d,\mathbf{F}_{d},\alpha,\beta,\gamma_{\alpha},\gamma_{\beta},\mathbf{\Omega})
\end{equation}
representing the controller. As can be seen the controller requires as input among the meta-parameters and the percept vector $\Omega$ only a desired velocity and a feed-forward wrench. Note that the desired velocity can integrated into a desired pose and compared to the current pose provided by $\Omega$ to acquire the motion error.

\subsection{Manipulation Skill}\label{sec:pd_skill}

A manipulation skill is defined as the directed graph $G$ consisting of nodes $N$ and transitions $T$. A node $n \in N$ is also called a manipulation primitive (MP) while an edge $e \in E$ is also called a transition. The transitions are activated by conditions that mark the success of the preceding MP. A single MP consists of a parameterized velocity and force trajectory.

\subsubsection{Directed Skill Graph}

Figure \ref{fig:skill} shows a principle depiction of $G$. We add an additional initial node and a terminal node. The transition coming from the initial node is triggered by the \textit{precondition} while the transition leading to the terminal node is activated by the \textit{success condition}. Furthermore, every MP has an additional transition that is activated by an \textit{error condition} and leads to a recovery node. Note, the presented structure could also be described as a hierarchical statemachine if everything between the initial and terminal node is considered a single state consisting of a number of child states.

Although it is possible we do not consider backwards directed transitions in this work since we intend to find a solution that is able 

\begin{figure}
\begin{center}
\input{fig_skill_01.pdf_tex}
\caption{Skill graph $G$.}
\label{fig:skill}
\end{center}
\end{figure}

Lastly, a learning metric is used to evaluate the skill execution in terms of a success indicator and a predefined cost function.

\subsubsection*{Conditions}

There are three condition types involved in the execution of skills: preconditions $\mathcal{C}_\text{pre}$, failure conditions $\mathcal{C}_\text{err}$ and success conditions $\mathcal{C}_\text{suc}$. They all share the same basic definition, yet their application is substantially different. Their purpose is to define the borders and limits of the skill from start to end.

\begin{definition}[Condition]
Let $\mathcal{C} \subset \mathsf{S}$ be a closed set and $\mathsf{c}(\mathbf{X}(t))$ a function $\mathsf{c}: \mathcal{S}\rightarrow \mathbb{B}$ where $\mathbb{B}=\{0,1\}$. A condition holds iff $\mathsf{c}(\mathbf{X}(t))=1$. Note that the mapping itself obviously depends on the specific type of condition.
\end{definition}

\begin{definition}[Precondition]
$\mathcal{C}_{pre}$ denotes the chosen set for which the precondition defined by $\mathsf{c}_{pre}(\mathbf{X}(t))$ holds. The condition holds, i.e. $\mathsf{c}_{pre}(\mathbf{X}(t_0))=1$, iff $\forall \; x \in \mathbf{X}: x(t_0) \in \mathcal{C}_{pre} $. $t_0$ denotes the time at start of the skill execution.
\end{definition}

\begin{definition}[Error Condition]
$\mathcal{C}_{err}$ denotes the chosen set for which the error condition $\mathsf{c}_{err}(\mathbf{X}(t))$ holds, i.e. $\mathsf{c}_{err}(\mathbf{X}(t))=1$. This follows from $\exists \; x \in \mathbf{X}: x(t) \in \mathcal{C}_{err} $.
\end{definition}

\begin{definition}[Success Condition]
$\mathcal{C}_{suc}$ denotes the chosen set for which the success condition defined by $\mathsf{c}_{suc}(\mathbf{X}(t))$ holds, i.e. $\mathsf{c}_{suc}(\mathbf{X}(t))=1$ iff $\forall x \in \mathbf{X}: x(t) \in \mathcal{C}_{suc} $.
\end{definition}

The precondition states the conditions under which the skill can be initialized. The error condition stops the execution when fulfilled and returns a negative result. The success condition determines when the execution was successful. Note, that we also make use of the definition of the success condition to describe the transitions between MPs.

\subsubsection*{Evaluation}

\begin{definition}[Learning Metric]
$\mathcal{Q}$ denotes the set of all $2-$tuples $(w,f_q(\mathbf{X}(t))$ with $0<w<1$ and the result indicator $r=\{0,1\}$ where $0$ means failure and $1$ success. 
Let $q=\sum_i w_i f_{q,i}(\mathbf{X}(t)) \;\forall \; (w_i,f_{q,i}(\mathbf{X}(t))) \in \mathcal{Q}$ be the cost function of the skill.
\end{definition}

\subsubsection{Manipulation Primitive}

The motion and interaction commands to be executed in node $n \in N$ of $G$ are defined as

\begin{align*}
\dot{\mathbf{x}}_{d} &= f_{t}(\mathbf{P}_{t},\mathbf{p}_s)\\
\mathbf{F}_{d} &= f_{w}(\mathbf{P}_{w},\mathbf{p}_s)
\end{align*}

where $\dot{\mathbf{x}}_{d}$ is the desired twist and $\mathbf{F}_{d}$ the feed forward wrench commanded by the skill when the node $n$ is active. These commands are described with respect to a task frame $TF$. $\mathbf{p}_s$ is the vector of robot percepts.
$\mathbf{p}_{t}$ is the set of parameters used by node $n$ to generate twist commands while $\mathbf{p}_{w}$ is used to generate the wrench commands. Moreover, $\mathbf{p}_{t} \subset \mathcal{P}$ and $\mathbf{p}_{w} \subset \mathcal{P}$ where $\mathcal{P}$ is the set of all parameters.

Furthermore, we divide $\mathcal{P}$ into two subsets $\mathcal{P}_l$, which is the subset of all parameters that are to be learned, and $\mathcal{P}_c$ which contains all other parameters that are determined by the context of the task.
The parameters in $\mathcal{P}_l$  are chosen from a domain $\mathcal{D}$ which is also determined by the task context or system capabilities.

When a transition is activated and the commands are switched from node $n_i$ to $n_{i+1}$ the switching behavior should be regulated. This could for example be achieved by limiting the derivative of the commands.

\subsubsection{Peg-in-Hole}

In the following the peg-in-hole skill is described by applying the formalism above. Figure shows the graph of the skill including the manipulation primitives. In Tab. all parameters $p \in \mathcal{P}$ used by the peg-in-hole skill are listed.

\begin{figure*}
\begin{center}
\input{fig_peginhole.pdf_tex}
\caption{Depiction of the peg-in-hole skill graph.}
\label{fig:peginhole}
\end{center}
\end{figure*}

\renewcommand{\arraystretch}{1.3}
\begin{table}
\begin{center}
\begin{tabular}{|p{1.5cm}|p{6cm}|}
\hline 
Parameter & Description \\ 
\hline 
$T_\text{h}$ & The estimated hole pose \\
\hline 
ROI & Region of interest around the hole \\
\hline 
$d$ & Depth of the hole \\
\hline 
$\dot{\mathbf{x}}_\text{max}$ & Maximum allowed velocity for translation and rotation\\
\hline
$\ddot{\mathbf{x}}_\text{max}$ & Maximum acceleration for translation and rotation\\
\hline
$\varphi_\text{init}$ & Initial tilt of the object relative to the hole \\
\hline
$f_\text{c}$ & Contact force between robot and environment \\
\hline 
$s$ & Speed factor \\
\hline 
$a_t$ & Amplitude of translational wiggle motion \\
\hline
$a_r$ & Amplitude of rotational wiggle motion \\
\hline
$\omega_t$ & Frequency of translational wiggle motion \\
\hline
$\omega_r$ & Frequency of rotational wiggle motion \\
\hline
\end{tabular} 
\end{center}
\end{table}

\subsubsection*{Conditions}

\begin{itemize}
\item $\mathcal{C}_{pre}=\{\mathbf{X} | T \in U(T_\text{a}),g=1\}$ states that the robot is within an environment $U$ of the approach pose $T_\text{a}$ which is slightly above $T_h$ and tilted by $\varphi_\text{init}$. The variable $g \in \mathbf{X}$ indicates whether the robots has grasped something or not.
\item $\mathcal{C}_{suc}=\{\mathbf{X} | T_z >T_{h,z}+d\}$ which states that the object has to be inserted by at least the distance $d$ into the hole for the skill to terminate successfully. Ideally, $d$ is the depth of the hole.
\item $\mathcal{C}_{err}=\{\mathbf{X} |  T \notin \text{ROI},{\boldsymbol{\tau}}_{ext}>\V{\tau}_{max},t>t_\text{max}\}$ states that the skill fails if the robot leaves the region of interest (ROI) around the hole, the external torques exceed component wise some specified safety limit or the maximum time is exceeded.
\end{itemize}

\subsubsection*{Transitions}

The transitions of the peg-in-hole skill are defined as follows.

\begin{itemize}
\item $e_1$, reached end of approach trajectory
\item $e_2$, $f_c$ is exceeded in z-direction
\item $e_3$, $f_c$ is exceeded in x-direction
\item $e_4$  reached end of alignment trajectory
\end{itemize}

\subsubsection*{Manipulation Primitives}

The MPs are defined as follows:
\begin{itemize}
\item $n_1$: The robot moves to the approach pose above the hole.
\begin{equation}
\dot{\mathbf{x}}_{d}=f_\text{p2p}(T_\text{a},s \dot{\mathbf{x}}_\text{max},\ddot{x}_\text{max},), \; \mathbf{F}_{d}=\mathbf{0}
\end{equation}
$f_\text{p2p}$ generates a trapezoidal velocity profile to move from the current pose to a goal pose while considering a given velocity and acceleration.
\item $n_2$: The robot moves towards the surface with the hole and establishes contact.
\begin{equation}
\dot{\mathbf{x}}_{d}=\left[\begin{array}{cccccc}
0 & 0 & s \dot{\mathbf{x}}_\text{max} & 0 & 0 & 0
\end{array}\right]^T,\;\mathbf{F}_{d}=\mathbf{0}
\end{equation}
\item $n_3$: The object is fit into the holes geometry.
\begin{equation}
\dot{\mathbf{x}}_{d}=\left[\begin{array}{cccccc}
s \dot{\mathbf{x}}_\text{max} & 0 & 0 & 0 & 0 & 0
\end{array}\right]^T,\;\mathbf{F}_{d}=\left[\begin{array}{cccccc}
0 & 0 & f_\text{c} & 0 & 0 & 0
\end{array}\right]^T
\end{equation}
\item $n_4$: The object is rotated into the estimated orientation of the hole while holding contact between object and hole.
\begin{equation}
\dot{\mathbf{x}}_{d}=f_\text{p2p}(T_\text{h},s \dot{\mathbf{x}}_\text{max},\ddot{\mathbf{x}}_\text{max}), \; \mathbf{F}_{d}=\left[\begin{array}{cccccc}
f_\text{c} & 0 & f_\text{c} & 0 & 0 & 0
\end{array}\right]^T
\end{equation}
\item $n_5$: The object is inserted into the hole.
\begin{equation}
\dot{\mathbf{x}}_{d}=\left[\begin{array}{cccccc}
a_t \sin(2\pi \omega_t) & a_t \sin(2\pi \frac{3}{4}\omega_t) & s \dot{\mathbf{x}}_\text{max} & a_r \sin(2\pi \omega_r) & a_r \sin(2\pi \frac{3}{4}\omega_r) & 0
\end{array}\right]^T,\;\mathbf{F}_{d}=\mathbf{0}
\end{equation}
\end{itemize}

